Resource optimization for fault-tolerant quantum computing

In this thesis we examine a variety of techniques for reducing the resources required for fault-tolerant quantum computation. First, we show how to simplify universal encoded computation by using only transversal gates and standard error correction procedures, circumventing existing no-go theorems. We then show how to simplify ancilla preparation, reducing the cost of error correction by more than a factor of four. Using this optimized ancilla preparation, we develop improved techniques for proving rigorous lower bounds on the noise threshold. Additional overhead can be incurred because quantum algorithms must be translated into sequences of gates that are actually available in the quantum computer. In particular, arbitrary single-qubit rotations must be decomposed into a discrete set of fault-tolerant gates. We find that by using a special class of non-deterministic circuits, the cost of decomposition can be reduced by as much as a factor of four over state-of-the-art techniques, which typically use deterministic circuits. Finally, we examine global optimization of fault-tolerant quantum circuits under physical connectivity constraints. We adapt techniques from VLSI in order to minimize time and space usage for computations in the surface code, and we develop a software prototype to demonstrate the potential savings.

==> qecc.tex <==
\chapter[Quantum error-correcting codes]{Quantum error-correcting codes\label{chap:qecc}}
\section{The Golay code\label{sec:golay-code}}

The Golay code is a perfect CSS $[[23,1,7]]$ quantum error-correcting code (see e.g.,~\cite{Steane2003}).  It has eleven $X$ and eleven $Z$ stabilizer generators.  The code is self-dual, and the $X$ and $Z$ stabilizer generators can both be given by the following eleven $23$-character strings: 
\begin{equation} \label{eq:golay-stabilizers}
\begin{tabular}{c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}c@{\:}}
. &1 &. &. &1 &. &. &1 &1 &1 &1 &1 &. &. &. &. &. &. &. &. &. &. &1\\
1 &. &. &1 &. &. &1 &1 &1 &1 &1 &. &. &. &. &. &. &. &. &. &. &1 &.\\
. &1 &1 &. &1 &1 &1 &. &. &. &1 &1 &. &. &. &. &. &. &. &. &1 &. &.\\
1 &1 &. &1 &1 &1 &. &. &. &1 &1 &. &. &. &. &. &. &. &. &1 &. &. &.\\
1 &1 &1 &1 &. &. &. &1 &. &. &1 &1 &. &. &. &. &. &. &1 &. &. &. &.\\
1 &. &1 &. &1 &. &1 &1 &1 &. &. &1 &. &. &. &. &. &1 &. &. &. &. &.\\
. &. &. &1 &1 &1 &1 &. &1 &1 &. &1 &. &. &. &. &1 &. &. &. &. &. &.\\
. &. &1 &1 &1 &1 &. &1 &1 &. &1 &. &. &. &. &1 &. &. &. &. &. &. &.\\
. &1 &1 &1 &1 &. &1 &1 &. &1 &. &. &. &. &1 &. &. &. &. &. &. &. &.\\
1 &1 &1 &1 &. &1 &1 &. &1 &. &. &. &. &1 &. &. &. &. &. &. &. &. &.\\
1 &. &1 &. &. &1 &. &. &1 &1 &1 &1 &1 &. &. &. &. &. &. &. &. &. &.
\end{tabular}
\end{equation}
Here, the $1$s in a row either all indicate $Z$ operators or all indicate $X$ operators, and dots indicate identity operators.  %\footnote{Our presentation is taken from~\cite{Reichardt2006}.}  
For example, the first line indicates that $I \otimes Z \otimes I \otimes I \otimes Z \otimes \cdots \otimes Z$ and $I \otimes X \otimes I \otimes I \otimes X \otimes \cdots \otimes X$ are stabilizers.  Note that each stabilizer generator has weight eight.  We index the qubits left to right, from $0$ to $22$.

The stabilizer generators partition the group of Pauli errors on $23$-qubits into $2^{24}$ cosets.  In particular, there are $2^{23-11}=2^{12}$ inequivalent $X$ errors (tensor products of $X$ and $I$) and $2^{12}$ inequivalent $Z$ errors (tensor products of $Z$ and $I$).

The Golay code is preserved by qubit permutations in a symmetry group known as the Mathieu group $M_{23}$.  %\footnote{This symmetry is inherited from the classical $23$-bit Golay code.  See, e.g.,~\cite{Huffman1998} pp.\ 1411.  Generators for this group can be obtained at~\cite{Gang}.}  
This is a four-transitive group of order $23 \cdot 22 \cdot 21 \cdot 20 \cdot 48$.  It is generated by a cyclic shift, and by the permutation 
$$
(2, 16, 9, 6, 8)(3, 12, 13, 18, 4)(7, 17, 10, 11, 22)(14, 19, 21, 20, 15)
\enspace,
$$
in cycle notation.  See~\cite[pp.~1411]{Huffman1998} and~\cite{Gang1999}.  


==> separate.tex <==
\chapter{Separating $X$ and $Z$ errors}
One of the multitude of reasons why CSS codes are convenient for use in fault-tolerance schemes is that $X$ errors and $Z$ errors may be corrected independently.  As a result, when analyzing error propagation through a quantum circuit, it is often sufficient to keep track of $X$ and $Z$ errors separately. 

Counting $X$ and $Z$ errors separately can lead to a dramatic reduction in complexity.  The number of inequivalent $X$ errors scales as $2^{n-n_X}$ and the number of inequivalent $Z$ errors scales as $2^{n-n_Z}$. Whereas the total number of inequivalent Pauli errors scales as $2^{n+k}$.  For codes that protect evenly against $X$ and $Z$ errors the improvement is roughly quadratic.

Unfortunately, in many noise models, $X$ and $Z$ are correlated.  In the depolarizing channel, for example, $X$ and $Z$ errors occur simultaneously as $Y$ errors one-third of the time. If the error-correction procedure is deterministic, then marginal probabilities can be used to obtain accurate statistics.  But if error \emph{detection} is used, as in ancilla verification, then separately tracking $X$ and $Z$ will yield higher undetected error rates.

For example, suppose we use a distance-$3$ CSS code.  Then the error $XXY$ is detectable by measuring the $X$ stabilizers.  But when counting $X$ and $Z$ separately, the above error splits into $XXX$ and $IIZ$ parts.  The $IIZ$ error can still be detected, but the $XXX$ error must be pessimistically considered undetectable.

Nonetheless, so long as $Y$ errors occur with about the same probability as $X$ and $Z$ alone, then separately counting $X$ and $Z$ can still be a good choice. 
Indeed, for the Golay code, counting $X$ and $Z$ errors simultaneously is highly impractical. On each $23$-qubit code block, there are $2^{12}$ inequivalent $X$ errors and $2^{12}$ inequivalent $Z$ errors, and thus $2^{24}$ inequivalent Pauli errors total.  (For example, there are $2^{23}$ different tensor products of $X$ and $I$ operators, and the group of $X$ stabilizers has size $2^{11}$, leaving $2^{12}$ $X$-error equivalence classes.)  For a rectangle involving two code blocks, this means we should compute for each~$k$ up to $(2^{24})^4$ quantities, one for each combination of input and output errors.  Counting $X$ and $Z$ errors separately yields a far more manageable $2\cdot (2^{12})^4=2^{49}$ combinations.

Standard malignant set counting does not treat $X$ and $Z$ errors separately, primarily because bounds on specific types of errors are not inherently preserved under level reduction.  \secref{sec:} discusses a method for circumventing this limitation.
\todo{Explain more here, but leave specifics for later sections.}

\begin{itemize}
  \item Cases in which $X$ and $Z$ cannot be tracked independently.
\end{itemize} 

